Directional Multivariate Ranking

User-provided multi-aspect evaluations manifest users' detailed feedback on the recommended items and enable fine-grained understanding of their preferences. Extensive studies have shown that modeling such data greatly improves the effectiveness and explainability of the recommendations. However, as ranking is essential in recommendation, there is no principled solution yet for collectively generating multiple item rankings over different aspects. In this work, we propose a directional multi-aspect ranking criterion to enable a holistic ranking of items with respect to multiple aspects. Specifically, we view multi-aspect evaluation as an integral effort from a user that forms a vector of his/her preferences over aspects. Our key insight is that the direction of the difference vector between two multi-aspect preference vectors reveals the pairwise order of comparison. Hence, it is necessary for a multi-aspect ranking criterion to preserve the observed directions from such pairwise comparisons. We further derive a complete solution for the multi-aspect ranking problem based on a probabilistic multivariate tensor factorization model. Comprehensive experimental analysis on a large TripAdvisor multi-aspect rating dataset and a Yelp review text dataset confirms the effectiveness of our solution.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts
		


==> intro_backup_2-8.tex <==
\section{Introduction}
\label{sec:intro}
Multi-aspect user evaluation of the items provides more informative feedback than merely overall evaluations. For better recommendations, such fine-grained feedback has been massively collected and studied to comprehend users' in-depth preferences. Extensive studies on modeling such detailed user feedback have shown promising results in predicting user's fine-grained aspect-level preferences in modern recommender systems \cite{viewpoint, EFM, bptf, Multi-sideTF}. %However, most of them focus on point-wise predictions of aspect-level preferences, and fail to realize the dependence between aspects. 

Recommendation is essentially a \emph{ranking} problem \cite{Sun2017MRLRMR,MTER}; and multi-aspect preferences shed light on more holistic and insightful item rankings. %In addition to enhancing the overall ranking with aspect-level preferences, 
Being able to provide multiple rankings with respect to different aspects elevates a user's freedom in interacting with the recommended items \cite{aspectrec}. For example, in hotel recommendation, a user may prefer to rank the items by the aspect of \textit{Value} that he/she cares mostly, while another user may choose to rank by \textit{Service} or a simple combination of a few aspects. Existing ranking solutions, such as %matrix factorization \cite{Koren:2009:MFT:1608565.1608614} or 
Bayesian personalized ranking (BPR) \cite{BPR}, are only designed for single-aspect ranking. They isolate the aspects, thus fail to realize the dependence among them for mutually enhancing the ranking performance under each aspect. For instance, \textit{Value} and \textit{Service} might be correlated in a user's evaluation of hotels; but if one simply estimates two separate rankers for these two aspects from the user's past evaluations, such \emph{personalized} correlation cannot be exploited or maintained in ranking new hotels for this user. 

The fundamental research question in multi-aspect recommendation, i.e., \textit{how to generate multiple rankings with respect to different aspects collectively}, remains under-explored. One possible solution is to apply multi-task learning \cite{RMTL, MTER}
%multi-objective optimization \cite{wei-MOO}
to learn a shared set of parameters that govern the rankings in multiple aspects.
%, where each aspect contributes to a separate ranking loss. 
But as it decomposes the multi-aspect ranking problem into multiple single aspect ranking sub-tasks and simply joins them with parameter sharing, there is no guarantee that the ranking on different aspects will correlate with each other. Arguably, users' evaluations on multiple aspects are dependent and compose a holistic assessment of the item \cite{aspectrec,MTER}; and thus they should be organically modeled for jointly improved ranking performance over aspects. 
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.96\linewidth]{figures/review_pair.pdf}
    \caption{Multi-aspect evaluations on two hotels from the same user on TripAdvisor.}
    \label{fig:review}
    %\vspace{-1em}
\end{figure}

Another challenge in ranking multiple aspects collectively lies in constructing the comparison between a pair of items.
%as well as to maintain the dependence among aspects. 
In single aspect ranking, the pair-wise order can be directly obtained by the result of binary comparisons \cite{BPR,l2r}, e.g., a five-star item is better than a three-star one. Nevertheless, in the multi-aspect scenario, the order between two items is \textit{multifaceted}, where the result of cross aspect comparison carries users' implicit emphasis over these aspects. %This should be captured and realized when recommending new items to the users. 
For instance, Figure \ref{fig:review} shows a pair of multi-aspect evaluations from the same user on two hotels selected from TripAdvisor. %\footnote{https://www.tripadvisor.com/}. %Besides the overall rating, the user also rated multiple specific aspects such as \textit{Rooms} and \textit{Location}. 
Although the first hotel receives a higher rating on the \textit{Value} aspect from the user, it gets a lower rating on \textit{Service}. Moreover, the difference on \textit{Value} is one star, while it is a three-star difference on \textit{Service}, which reflects the relative significance of the pair-wise comparison on these two aspects for this user. Intuitively, an aspect of three-star difference should be emphasized more than that with a one-star difference, when jointly optimizing the ranking over multiple aspects. In other words, the aspect with a more significant pairwise comparison result (3-star difference on the two items) should has a higher weight than the aspect with a weak pairwise comparison result (1-star difference) in the joint ranking objective.
%the relative significance across aspects in ranking these two hotels should be recognized and maintained in the learnt item rankings. 
%Thus such comparison significance is useful to signify the relative importance of the pair-wise order on an aspect in the collective ranking objective.  
Therefore, we require the constructed pair-wise order on multi-aspect preferences to embed two folds of information: 
\begin{enumerate*}[label=(\roman*)]
  \item the single-aspect orders on each aspect; and
  \item the relative significance of the comparison results on each aspect.
\end{enumerate*}

%In the single aspect comparison, the order can be alternatively perceived as the sign of the difference between two scalar evaluations. 
%Based on the vectorized representations for multi-aspect evaluations, 
%In any valid Euclidean space, each point represents a vector from the origin to itself. Our key insight is that the direction from one point to the other point can be adopted as the pair-wise comparison signal between two vectors.
%In order to model multiple aspect user feedback as an integrated evaluation, 
To provide a unified criterion for multi-aspect ranking, we take a vectorized representation of users' multi-aspect evaluation on each item and explicitly model the dependency across aspects. Specifically, the vectorized representations of the multi-aspect evaluations on two items naturally enables us to encode the single-aspect orders as well as relative significance of comparison across aspects
%Hence, each observation is considered as a vector in the multi-aspect preference space. %Our key insight is that the pair-wise order between two preference vectors can be defined 
in the \emph{direction} of their pairwise difference vector. To be more concrete, for each element in the difference vector, the sign of this element provides the pairwise order on the corresponding aspect; and the \emph{relative} absolute value indicates the significance of the pairwise comparison of this aspect. %Later in Section \ref{sec:method}, we prove that it satisfies the two-fold information needs. %where the direction can capture both the single-aspect orders and the relative significance of each aspect's comparison. 
%It worth mentioning that 
More importantly, for each aspect, only the pairwise order matters for ranking. Rather than recovering the exact difference vector as in a conventional regression problem, we look for methods that maintain the observed direction of the difference vector, regardless of the magnitude. This gives rise to the need of directional analysis of the difference vector: the multi-aspect ranking criterion can thus be formulated as learning a joint ranking function (i.e., across aspects) that maximizes the likelihood of the observed pair-wise directions. A potential solution can be acquired from directional statistics \cite{Bahlmann:2006:DFO:1220964.1221165}, which impose probability distributions for modeling the difference vector as a circular variable  \cite{SphereDispersion}. %such as von Mises-Fisher distribution \cite{SphereDispersion}.
Nonetheless, they are often limited to normalized magnitude and are not able to model the dependence among dimensions. 

We devise our new directional statistics to define the ranking criterion. Specifically, we compute likelihood of the observed directions under a ranking model by taking \emph{line integral} along the directions over the model's imposed distribution of pairwise difference vectors. The ranking model is thus optimized by maximizing this likelihood. We refer to this new ranking criterion as Directional Multivariate Ranking, or DMR in short. %Maximizing the likelihood over all observed pair-wise directional orders then becomes our criterion for multi-aspect ranking.
%To support this new ranking criterion,
We further apply the developed criterion to a probabilistic multivariate tensor factorization model (PMTF), which enables probabilistic assessment of multi-aspect comparisons. The personalized dependency among aspects can be modeled via personalized covariance matrices in PMTF, e.g., imposing a multivariate Gaussian distribution over the generation of preference vectors for a specific user. In this work, we focus on probabilistic tensor factorization for completing the solution. But the proposed ranking criterion is generally applicable to a much broader scope of ranking models, as long as they can define a probability distribution of the pairwise difference vector, such as deep neural network based models \cite{NCF}. 

%Importantly, the dependence within multiple aspects is indispensable in modeling. For example, the ratings on aspect \textit{Value} and \textit{Room} tend to be similar and correlated in Figure \ref{fig:review}, which imposes certain consistence of the pair-wise comparisons on these two aspects. To satisfy these requirements, we propose 
%as sampling from a \textit{multivariate} Gaussian distribution. We complete the solution for multi-aspect ranking by deriving the explicit ranking objective with the probabilistic modeling.

\begin{comment}
Instead, fomally derive the likelihood of the observed direction by taking line integral along the direction over the distribution of the difference vector. For supporting the ranking criterion, a probabilistic description of the observed multi-aspect evaluations is needed. 
%There is rich literature in user's preference prediction \cite{Koren:2009:MFT:1608565.1608614, multiverse, jmars} where real positive ratings are used to represent the preference levels. The probability is obtained from the preference levels by simply using a link function such as sigmoid \cite{BPR} or softmax \cite{Sun2017MRLRMR}, which will confound all aspects and lose the important dependence among them.
Specifically, we are committed to a flexible probabilistic modeling of multi-aspect preferences that enables the direct comparison between vectors. Moreover, the dependence within multiple aspects is indispensable. For example, in Figure \ref{fig:review}, the ratings on aspect \textit{Value} and \textit{Room} tend to be similar and correlated, which imposes certain consistence of the comparisons on these two aspects. Among various preference modeling methods, tensor factorization has proved its natural fitness and flexibility in modeling multi-aspect data \cite{TensorDecomp, MTER, multiverse, tagRec}. %Concretely, probabilistic tensor factorization based methods \cite{bptf, Rai:2015:SPT:2832747.2832775} are introduced to model the generation of multi-aspect data. 
However, almost all previous TF-based methods model users' preferences over multiple aspects as independent, by defining the likelihood of observing multi-aspect preferences as a point-wise product of each aspect \cite{Rai:2015:SPT:2832747.2832775, bptf, temporal}. %As a result, the dependence among multiple aspects is ignored. 
Instead, we propose a probabilistic multivariate tensor factorization method (PMTF) for modeling the generation of multi-aspect rating vectors as sampling from a multivariate Gaussian distribution. %The dependence among aspects is explicitly introduced in PMTF by the covariance matrices. This new perspective enables the ranking of multiple aspects collectively in a multivariate fashion, as well as making it possible to provide correlation based aspect-level explanations.
\end{comment}

To evaluate the multi-aspect ranking performance of the proposed solution, we collected a large hotel multi-aspect rating dataset from TripAdvisor. As reviews are common and abundant aspect-level evaluations can be extracted \cite{EFM,lara}, we also utilize a Yelp review dataset to verify our method's generalization to the review data. Extensive experiment comparisons against several baselines demonstrate the effectiveness of our proposed solution.

In the rest of the paper, we introduce the related work in Section \ref{sec:related}. In Section \ref{sec:method}, we first develop the multi-aspect ranking criterion step by step, leading to the DMR criterion in Eq~\eqref{eq:dmr}; and then we complete the solution with a probabilistic multivariate tensor factorization model. We conduct comprehensive experiment analysis of the proposed solution in Section \ref{sec:exp} and summarize the paper in Section \ref{sec:conclusion}.

%\nan{Shall we put a paragraph here for contributions?}

%Further empirical analysis on the ranking criterion and the introduction of the correlations among aspects shows the rationale and advantages of our design.
%The contributions of this work are as follows. First, by defining the directional order in the multi-aspect case and dependence among aspects, our solution organically incorporates the aspect-level comparisons for enhancing the overall ranking. Second, as the directional order captures the single-aspect orders on all aspects, we are able to provide multiple rankings based on different aspects, which promotes user's freedom in ranking items. Experiment results on a large hotel multi-aspect rating dataset from TripAdvisor and a Yelp review dataset demonstrate the effectiveness of our solution.

%We collected a large hotel multi-aspect rating dataset from TripAdvisor to evaluate the multi-aspect ranking performance of the proposed solution. As reviews are common and abundant aspect-level evaluations can be extracted \cite{EFM,MTER,lara}, we also utilize a Yelp review dataset to verify our method's generalization to the review data. Extensive experiment comparisons against several baseline multi-aspect preference modeling methods demonstrate the effectiveness of our proposed solution on the multi-aspect ranking task. %Further empirical analysis on the ranking criterion and the introduction of the correlations among aspects shows the rationale and advantages of our design.


==> intro_backup_2-9.tex <==
\section{Introduction}
\label{sec:intro}
Users' multi-aspect evaluation of items provides more informative feedback than merely an overall evaluation. For better recommendations, such fine-grained feedback has been massively collected and studied to comprehend users' in-depth preferences. Extensive studies on modeling such detailed user feedback have shown promising results in predicting user's fine-grained aspect-level preferences in modern recommender systems \cite{viewpoint, EFM, bptf, Multi-sideTF}. %However, most of them focus on point-wise predictions of aspect-level preferences, and fail to realize the dependence between aspects. 

Recommendation is essentially a \emph{ranking} problem \cite{Sun2017MRLRMR,MTER}; 
%and multi-aspect preferences shed light on more holistic and insightful item rankings. %In addition to enhancing the overall ranking with aspect-level preferences, 
%Being able to 
and providing multiple rankings with respect to different aspects elevates a user's freedom in interacting with the recommended items \cite{aspectrec}. For example, in hotel recommendation, a user may prefer to rank hotels by the aspect of \textit{Value} that he/she cares mostly, while others may choose to rank by \textit{Service} or a simple combination of a few aspects. 

Arguably, users' evaluations on multiple aspects are dependent and compose a holistic assessment of an item \cite{aspectrec,MTER}; and they should be organically modeled for jointly improved ranking performance over aspects. Thus in multi-aspect ranking, a ranking algorithm should generate \emph{structured} rating predictions for each user-item pair on all aspects, which can be then used for ranking on each aspect. However, most existing ranking solutions, such as Bayesian personalized ranking (BPR) \cite{BPR}, are only designed for single-aspect ranking. They isolate the aspects, thus fail to realize the dependence among them for mutually enhancing the ranking performance under each aspect. For instance, \textit{Value} and \textit{Service} might be correlated in users' evaluations of hotels; but if one simply estimates two separate rankers for these two aspects, such correlation cannot be exploited or maintained. Moreover, this correlation should be \emph{personalized}, e.g., different users correlate the aspects in different ways. This makes multi-aspect even more challenging. The fundamental research question in multi-aspect recommendation, i.e., \textit{how to generate multiple rankings with respect to different aspects collectively}, remains under-explored. One possible solution is to apply multi-task learning \cite{RMTL, MTER} to learn a shared set of parameters that govern the rankings in multiple aspects. But as it decomposes the multi-aspect ranking problem into multiple single aspect ranking sub-tasks and simply joins them with parameter sharing, there is no guarantee that the ranking on different aspects will correlate with each other. 
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.96\linewidth]{figures/review_pair.pdf}
    \caption{Multi-aspect evaluations on two hotels from the same user on TripAdvisor.}
    \label{fig:review}
    %\vspace{-1em}
\end{figure}

The challenge in ranking multiple aspects collectively while maintaining the structured dependence among aspects lies in constructing the comparison between a pair of items, which is non-trivial and less studied previously.
%as well as to maintain the dependence among aspects. 
In single aspect ranking, the pairwise order can be directly obtained by the result of binary comparisons \cite{BPR,l2r}, e.g., a five-star item is better than a three-star one. Nevertheless, in the multi-aspect scenario, the order between two items is \textit{multifaceted}, where the result of cross aspect comparison carries users' implicit emphasis over these aspects. %This should be captured and realized when recommending new items to the users. 
For instance, Figure \ref{fig:review} shows a pair of multi-aspect evaluations from the same user on two hotels selected from TripAdvisor. %\footnote{https://www.tripadvisor.com/}. %Besides the overall rating, the user also rated multiple specific aspects such as \textit{Rooms} and \textit{Location}. 
Although the first hotel receives a higher rating on the \textit{Value} aspect from the user, it gets a lower rating on \textit{Service}. Moreover, the difference on \textit{Value} is one star, while it is a three-star difference on \textit{Service}, which reflects the relative significance of the pairwise comparison on these two aspects for this user. Intuitively, an aspect of three-star difference should be emphasized more than that with a one-star difference, when jointly optimizing the ranking over multiple aspects. In other words, the aspect with a more significant pairwise comparison result (3-star difference on the two items) should has a higher weight than the aspect with a weak pairwise comparison result (1-star difference) in the joint ranking objective.
%the relative significance across aspects in ranking these two hotels should be recognized and maintained in the learnt item rankings. 
%Thus such comparison significance is useful to signify the relative importance of the pairwise order on an aspect in the collective ranking objective.  
Therefore, we require the constructed pairwise order on multi-aspect preferences to embed two folds of information: 
\begin{enumerate*}[label=(\roman*)]
  \item the single-aspect orders on each aspect; and
  \item the relative significance of the comparison results on each aspect.
\end{enumerate*}

%In the single aspect comparison, the order can be alternatively perceived as the sign of the difference between two scalar evaluations. 
%Based on the vectorized representations for multi-aspect evaluations, 
%In any valid Euclidean space, each point represents a vector from the origin to itself. Our key insight is that the direction from one point to the other point can be adopted as the pairwise comparison signal between two vectors.
%In order to model multiple aspect user feedback as an integrated evaluation, 
To provide a unified criterion for multi-aspect ranking, we take a vectorized representation of users' multi-aspect evaluation on each item and explicitly model the dependency across aspects. Specifically, the vectorized representation of the multi-aspect evaluations on two items naturally enables us to encode the single-aspect orders as well as relative significance of comparison across aspects
%Hence, each observation is considered as a vector in the multi-aspect preference space. %Our key insight is that the pairwise order between two preference vectors can be defined 
in the \emph{direction} of their pairwise difference vector. To be more concrete, for each element in the difference vector, the sign of this element provides the pairwise order on the corresponding aspect; and the ratio between them indicates the significance of the pairwise comparison of this aspect. %Later in Section \ref{sec:method}, we prove that it satisfies the two-fold information needs. %where the direction can capture both the single-aspect orders and the relative significance of each aspect's comparison. 
%It worth mentioning that 
More importantly, for each aspect, only the pairwise order matters for ranking. Rather than recovering the exact difference vector as in a conventional regression problem, we look for methods that maintain the observed direction of the difference vector, regardless of the magnitude. This gives rise to the need of directional analysis of the difference vector: the multi-aspect ranking criterion can thus be formulated as learning a joint ranking function (i.e., across aspects) that maximizes the likelihood of the observed pairwise directions. A potential solution can be acquired from directional statistics \cite{Bahlmann:2006:DFO:1220964.1221165}, which impose probability distributions for modeling the difference vector as a circular variable  \cite{SphereDispersion}. %such as von Mises-Fisher distribution \cite{SphereDispersion}.
Nonetheless, they are often limited to normalized magnitude and are not able to model the dependence among dimensions. 

We devise our new directional statistics to define the ranking criterion. Specifically, we compute likelihood of the observed directions under a ranking model by taking \emph{line integral} along the directions over the model's imposed distribution of pairwise difference vectors. The ranking model is thus optimized by maximizing this likelihood. We refer to this new ranking criterion as Directional Multivariate Ranking, or DMR in short. %Maximizing the likelihood over all observed pairwise directional orders then becomes our criterion for multi-aspect ranking.
%To support this new ranking criterion,
We further apply the developed criterion to a probabilistic multivariate tensor factorization model (PMTF), which enables probabilistic assessment of multi-aspect comparisons. The personalized dependency among aspects can be modeled via personalized covariance matrices in PMTF, e.g., imposing a multivariate Gaussian distribution over the generation of preference vectors for a specific user. In this work, we focus on probabilistic tensor factorization for completing the solution. But the proposed ranking criterion is generally applicable to a much broader scope of ranking models, as long as they can define a probability distribution of the pairwise difference vector, such as deep neural network based models \cite{NCF}. 

%Importantly, the dependence within multiple aspects is indispensable in modeling. For example, the ratings on aspect \textit{Value} and \textit{Room} tend to be similar and correlated in Figure \ref{fig:review}, which imposes certain consistence of the pairwise comparisons on these two aspects. To satisfy these requirements, we propose 
%as sampling from a \textit{multivariate} Gaussian distribution. We complete the solution for multi-aspect ranking by deriving the explicit ranking objective with the probabilistic modeling.

\begin{comment}
Instead, fomally derive the likelihood of the observed direction by taking line integral along the direction over the distribution of the difference vector. For supporting the ranking criterion, a probabilistic description of the observed multi-aspect evaluations is needed. 
%There is rich literature in user's preference prediction \cite{Koren:2009:MFT:1608565.1608614, multiverse, jmars} where real positive ratings are used to represent the preference levels. The probability is obtained from the preference levels by simply using a link function such as sigmoid \cite{BPR} or softmax \cite{Sun2017MRLRMR}, which will confound all aspects and lose the important dependence among them.
Specifically, we are committed to a flexible probabilistic modeling of multi-aspect preferences that enables the direct comparison between vectors. Moreover, the dependence within multiple aspects is indispensable. For example, in Figure \ref{fig:review}, the ratings on aspect \textit{Value} and \textit{Room} tend to be similar and correlated, which imposes certain consistence of the comparisons on these two aspects. Among various preference modeling methods, tensor factorization has proved its natural fitness and flexibility in modeling multi-aspect data \cite{TensorDecomp, MTER, multiverse, tagRec}. %Concretely, probabilistic tensor factorization based methods \cite{bptf, Rai:2015:SPT:2832747.2832775} are introduced to model the generation of multi-aspect data. 
However, almost all previous TF-based methods model users' preferences over multiple aspects as independent, by defining the likelihood of observing multi-aspect preferences as a point-wise product of each aspect \cite{Rai:2015:SPT:2832747.2832775, bptf, temporal}. %As a result, the dependence among multiple aspects is ignored. 
Instead, we propose a probabilistic multivariate tensor factorization method (PMTF) for modeling the generation of multi-aspect rating vectors as sampling from a multivariate Gaussian distribution. %The dependence among aspects is explicitly introduced in PMTF by the covariance matrices. This new perspective enables the ranking of multiple aspects collectively in a multivariate fashion, as well as making it possible to provide correlation based aspect-level explanations.
\end{comment}

To evaluate the multi-aspect ranking performance of the proposed solution, we collected a large hotel multi-aspect rating dataset from TripAdvisor. As reviews are common and abundant aspect-level evaluations can be extracted \cite{EFM,lara}, we also utilize a Yelp review dataset to verify our method's generalization to the review data. Extensive experiment comparisons against several baselines demonstrate the effectiveness of our proposed solution.

%In the rest of the paper, we introduce the related work in Section \ref{sec:related}. In Section \ref{sec:method}, we first develop the multi-aspect ranking criterion step by step, leading to the DMR criterion in Eq~\eqref{eq:dmr}; and then we complete the solution with a probabilistic multivariate tensor factorization model. We conduct comprehensive experiment analysis of the proposed solution in Section \ref{sec:exp} and summarize the paper in Section \ref{sec:conclusion}.

%\nan{Shall we put a paragraph here for contributions?}

%Further empirical analysis on the ranking criterion and the introduction of the correlations among aspects shows the rationale and advantages of our design.
%The contributions of this work are as follows. First, by defining the directional order in the multi-aspect case and dependence among aspects, our solution organically incorporates the aspect-level comparisons for enhancing the overall ranking. Second, as the directional order captures the single-aspect orders on all aspects, we are able to provide multiple rankings based on different aspects, which promotes user's freedom in ranking items. Experiment results on a large hotel multi-aspect rating dataset from TripAdvisor and a Yelp review dataset demonstrate the effectiveness of our solution.

%We collected a large hotel multi-aspect rating dataset from TripAdvisor to evaluate the multi-aspect ranking performance of the proposed solution. As reviews are common and abundant aspect-level evaluations can be extracted \cite{EFM,MTER,lara}, we also utilize a Yelp review dataset to verify our method's generalization to the review data. Extensive experiment comparisons against several baseline multi-aspect preference modeling methods demonstrate the effectiveness of our proposed solution on the multi-aspect ranking task. %Further empirical analysis on the ranking criterion and the introduction of the correlations among aspects shows the rationale and advantages of our design.


==> old_intro.tex <==
\section{Introduction}
\label{sec:intro}
To understand users' detailed preferences beyond merely their overall evaluations of an item, multi-aspect preferences are extensively collected and studied for better recommendation. For example, a user's ratings on different aspects, such as \textit{cleanliness}, \textit{location}, and \textit{service} of a hotel provide her detailed aspect-level preferences. Recommendation systems can take the advantage of such information to generate personalized aspect-level comparison and ranking across hotels based on the user's aspect emphasis \cite{lara}, e.g., recommending hotels not only by the predicted overall evaluation, but also by the cleanliness aspect that the user cares about. %Sometimes a user may also want to compare two items on different aspects. 
Moreover, previous studies show that incorporating multi-aspect preferences in addition to overall preference can greatly boost the performance of preference prediction, and also promote the explainability of the recommendation \cite{viewpoint, EFM, bptf, Hongimprove, fact}. Such performance improvement is usually achieved by jointly modeling multi-aspect preferences to learn better representations of users and items, and the aspect-level predictions are used as explanations. However, as recommendation is essentially a ranking problem \cite{MTER, Sun2017MRLRMR}, how to rank items with respect to multiple aspects collectively remains unsolved. Existing ranking criteria, such as Bayesian personalized ranking (BPR) \cite{BPR}, are only designed for single-aspect ranking. Therefore, they can only be applied to a single aspect or to each aspect independently as a multi-objective optimization problem \cite{wei-MOO}. We argue that multi-aspect preferences are a holistic evaluation and should be organically integrated for a joint ranking, where the key challenge is to define the orders of multi-aspect preferences and maintain their dependence. 
\begin{figure}
    \centering
    \includegraphics[width=0.96\linewidth]{figures/review_pair.png}
    \caption{Two multi-aspect evaluations on different hotels from the same user on TripAdvisor.}
    \label{fig:review}
    \vspace{-4mm}
\end{figure}

%Multi-aspect preferences compose a complete and detailed evaluation to an item. From the aspect level preferences, we can realize the reasons that a user likes or dislikes an item and provide recommendations based on detailed aspects. Multiple aspects preferences are usually correlated instead of being independent. For instance, the preference on a hotels room condition might be highly correlated with the cleanliness. Figure \ref{fig:review} shows a sample of hotel multi-aspect ratings on TripAdvisor. Besides the overall rating, the user also rated multiple specific aspects, which tells us how she likes different aspects of the hotel. And there are potential correlations between the aspects like \textit{`Value'} and \textit{`Service'}, \textit{`Rooms'} and \textit{`Cleanliness'}.

Figure \ref{fig:review} shows an example of multi-aspect evaluations from a user on two different hotels sampled from TripAdvisor\footnote{https://www.tripadvisor.com/}. Besides the overall rating, the user also rated multiple specific aspects such as \textit{Rooms} and \textit{Location}. From the aspect-level evaluations, we can realize how she likes each aspect of different hotels, e.g. although she gives a higher rating to \textit{Value} of the first hotel, she prefers the \textit{Location} of the second hotel. Moreover, the aspect evaluations are usually potentially correlated instead of being independent. For instance, the aspect \textit{Value} and \textit{Rooms} tend to have similar ratings. Our goal is to provide detailed and personalized comparison between different hotels on each specific aspect.   

In order to treat multi-aspect preferences a user shows to an item as an integrated evaluation, we first take a vectorized representation of the multi-aspect preferences. Therefore, each observation is defined as a vector of preferences over multiple aspects. However, unlike the simple binary comparison in the single-aspect case, how to define the order of two preference vectors remains intractable in the literature. Basically, we expect the multi-aspect order defined between vectors to capture the binary order on each aspect, as well as the relative significance of the comparison on each aspect against other aspects. Based on the vectorized representation, we consider the direction from one preference vector to another in the Euclidean space as the pair-wise comparison signal. The direction then serves as the pair-wise order proxy and contains both the single-aspect orders and the relative significance of each order. From this perspective, the pair-wise ranking criterion can be formulated as maximizing the likelihood of observing the direction from one vector to another. Rather than recovering the exact difference vector between two vectors, which is equivalent to point-wise estimation, the key is that we aim to maintain the observed direction between them, regardless of the magnitude. This gives rise to the need of directional analysis of the pair-wise difference between two rating vectors. Although directional statistics \cite{Bahlmann:2006:DFO:1220964.1221165} provides potential options for depicting the probability distribution of directions, such as von Mises-Fisher distribution \cite{SphereDispersion}, these distributions are often limited to normalized magnitude and are not able to model the dependence among dimensions. Instead, we derive the likelihood of the observed direction by taking line integral along the direction over the distribution of the difference vector. Maximizing the likelihood over all observed pair-wise orders then becomes our criterion for multi-aspect ranking.

For supporting the ranking criterion, we need a probabilistic description of the observed multi-aspect ratings. There is rich literature in user's preference prediction \cite{Koren:2009:MFT:1608565.1608614, multiverse, jmars} where real positive numbers are used to represent the preference level. The probability is obtained from the preference levels by simply using a link function such as sigmoid \cite{BPR} or softmax \cite{Sun2017MRLRMR}, which will confound all aspects and lose the important dependence among them. Instead, we are committed to a more specific and flexible probabilistic modeling of multi-aspect preferences that enables the direct comparison between vectors and maintains the dependence among aspects. Among all the preference modeling methods, tensor factorization has shown its natural fitness and effectiveness in modeling multi-aspect data \cite{TensorDecomp, MTER, multiverse, tagRec}. Specifically, probabilistic tensor factorization based methods \cite{bptf, Rai:2015:SPT:2832747.2832775} are introduced to model the generation of multi-aspect data. However, almost all previous TF-based methods model users' preferences over multiple aspects as independent, by defining the likelihood of observing multi-aspect preferences as a point-wise product of each aspect \cite{Rai:2015:SPT:2832747.2832775, bptf, temporal}. As a result, the dependence among multiple aspects is ignored. To explicitly capture the dependence among aspects, we propose a probabilistic multivariate tensor factorization method (PMTF) for modeling the generation of multi-aspect rating vectors as sampling from a multivariate Gaussian distribution. The dependency among aspects is explicitly introduced in PMTF by the covariance matrices. This new perspective makes it possible to model the intrinsic dependence among aspects, and such dependence also enables the ranking of multiple aspects collectively as well as aspect-based explanations of recommendations. 
%From an information-theoretic perspective \cite{l2x, Kullback1959Information}, we also show that by explicitly modeling the correlation, PMTF provides an information-theoretic regularization for the consistency and explainability of multi-aspect preference modeling. 

We collected a hotel multi-aspect rating dataset from TripAdvisor to evaluate the multi-aspect ranking performance of the proposed solution. As reviews are very common and abundant aspect-level evaluations can be extracted from reveiws \cite{EFM,MTER,lara}, we also utilize a Yelp review dataset to verify our method's generalization to the review data. Extensive experiment comparisons against several baseline multi-aspect preference modeling methods demonstrate the effectiveness of our proposed solution on the multi-aspect ranking task. Further empirical analysis on the ranking criterion and the introduction of the correlations among aspects shows the rationale and advantages of our design.



==> old_relatedwork.tex <==
\section{Related Works}
\label{sec:related}
Recommendation systems rely on the users' evaluations on items to learn their preferences and provide recommendations. Such evaluations are not unilateral, but \textit{multifaceted}. Understanding the detailed aspect-level evaluations may help us better comprehend their preferences and generate better recommendations \cite{DBLP:journals/corr/abs-1210-3926}. Extensive research effort has been devoted to incorporating the aspect-level preferences in addition to only overall preference \cite{jmars, lara, bptf, HFT}. Some of them also try to extract explicit aspect ratings from reviews based on sentiment analysis techniques when aspect-level ratings are not readily available \cite{EFM, MTER}. Empirical results show that the preference ranking and prediction performance can be significantly improved, by either jointly modeling multiple aspect preferences \cite{jmars, MTER} or use the aspect-level preferences as some regularization to learn better user/item representations \cite{fact, TEM}. Besides, another important benefit from introducing the aspect-level preferences is to improve the explainability of the recommendations by generating aspect-level explanations \cite{MTER, Multi-sideTF, fact}. 

As recommendation is essentially a ranking problem \cite{FactLambdamart,MTER}, personalized ranking criteria are proposed to directly optimize the ranking performance \cite{BPR, apr}. However, existing popular ranking criteria such as BPR are only designed for single-aspect ranking and usually applied to the overall preference to boost the ranking performance \cite{MTER, fact}. \cite{tagRec} applied BPR to rank different tags for a given user-item pair, but not to rank items with respect to different aspects. To the best of our knowledge, there is no principled solution for ranking multiple aspects collectively, which has great practical value in deployed recommendation systems. For example, a user may prefer to get recommendations based on some specific aspects, while pay less attention to other aspects. Sometimes users may also want to compare two items on different aspects. In order to provide personalized ranking and comparison on the detailed aspect-level, our proposed method aims to rank multiple aspects collectively. 

The key challenge in multi-aspect ranking is to view the aspect preferences a user gives an item as an integrated evaluation and define the order between two multi-aspect preference vectors. We propose to use the direction from one rating vector to another vector as the pair-wise order signal. %Therefore, directional descriptions between two preference vectors are necessary. 
Although there are distributions such as von Mises \cite{SphereDispersion} for modeling the vector as a circular variable \cite{batmanghelich-etal-2016-nonparametric}. They restrict the vector to a fixed magnitude and can not model the dependence among dimensions. \cite{mgvm} tries to generalize the von Mises distribution to the multivariate case to capture the correlations among dimensions. But it still lacks the flexibility of varying the magnitudes and depends on approximations without close-form analytic expression. We take a detour for getting the likelihood of the observed directions. For each pair-wise comparison, we first derive the density function of the difference vector, and then take the line integral along the observed direction. %In the next section, we will present the exact expression of the resulting likelihood and its tractability for optimization purpose.   

In order to complete the proposed solution for multi-aspect ranking and accord with the proposed ranking criterion, we seek supports from probabilistic tensor factorization methods \cite{bptf, Rai:2015:SPT:2832747.2832775}. Although tensor factorization is massively applied to multi-aspect data modeling \cite{TensorDecomp,pmf,temporal}, most previous works assume that the aspects are independent. Some of them directly apply tensor factorization methods to multi-aspect data \cite{multiverse, tensorrec}, which naturally disables the correlations among aspects. Others take a probabilistic perspective and explicitly define the likelihood of observing the preferences on multiple aspects as the point-wise product from each aspect preference \cite{temporal,bptf,Rai:2015:SPT:2832747.2832775}. As a result, the dependence among multiple aspects is ignored in modeling. To capture the dependence among aspects, we propose a probabilistic multivariate tensor factorization method (PMTF) for modeling the generation of aspect ratings as sampling from a \textit{multivariate} Gaussian distribution. %Based on this proposed method, we derive a directional probabilistic multivariate ranking solution (DPMR), which models the observed pair-wise orders of vectors in a multivariate fashion.  
